Circular economy meets building automation

This paper demonstrates the concept of reusing discarded smartphones to connect the end-of-life of e-wastes with the start-of-life of smart buildings. Two control-related and one communication-related case studies have been conducted experimentally to evaluate applicability. Diverse controlled systems, control tasks, and algorithms have been considered. In addition, the sufficiency of communication with external agents has been quantified. The proof-of-concept experiments indicate technical feasibility and applicability to typical tasks with satisfactory performance. As smartphones improve over time, higher computing performance and lower communication latency can be expected, enhancing the prospect of the proposed reuse concept.

==> sections/package_used.tex <==
% manage all package used
\usepackage{longtable}
\usepackage[nolist,printonlyused]{acronym}
\usepackage{rotating}
\usepackage[final]{pdfpages}
\usepackage{booktabs}
\usepackage{ltablex}
\usepackage{paralist}
\let\proof\relax
\let\endproof\relax
\usepackage{amsmath,empheq,amsthm,bm,tabularx}
\usepackage{acronym}
\usepackage[nocomma]{optidef}
\usepackage{color}
\usepackage{soul,xcolor}
\usepackage{pgfplotstable}
\usepackage{pgfplots}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{caption}
\usepackage{url}
\usepackage[official]{eurosym}
\usepackage{lineno}
\usepackage{longtable}
\usepackage{amssymb}
\usepackage{siunitx}
\usepackage{steinmetz}
\usepackage{tikz}
\usepackage[hidelinks]{hyperref}
\makeatletter
 \DeclareRobustCommand\ref{%
    \@ifstar\@refstar\T@ref
  }%
  \DeclareRobustCommand\pageref{%
    \@ifstar\@pagerefstar\T@pageref
  }%
 \makeatother
\usepackage{etoolbox}
\usepackage{booktabs}
\usepackage{subcaption}
\usetikzlibrary{arrows, chains, positioning, fit, quotes, shapes.geometric}
\usetikzlibrary{patterns}
\pagenumbering{arabic}

% \usepackage[a4paper,left=1in,right=1in, top = 0.7in]{geometry}
\usepackage{fancyhdr}
\usepackage[parfill]{parskip}
\usepackage{helvet}
\usepackage[printwatermark]{xwatermark}
%\newwatermark[allpages,color=gray!50,angle=45,scale=3,xpos=0,ypos=0]{CONFIDENTIAL\\DRAFT}
